Procedural Text Mining with Large Language Models

Recent advancements in the field of Natural Language Processing, particularly the development of large-scale language models that are pretrained on vast amounts of knowledge, are creating novel opportunities within the realm of Knowledge Engineering. In this paper, we investigate the usage of large language models (LLMs) in both zero-shot and in-context learning settings to tackle the problem of extracting procedures from unstructured PDF text in an incremental question-answering fashion. In particular, we leverage the current state-of-the-art GPT-4 (Generative Pre-trained Transformer 4) model, accompanied by two variations of in-context learning that involve an ontology with definitions of procedures and steps and a limited number of samples of few-shot learning. The findings highlight both the promise of this approach and the value of the in-context learning customisations. These modifications have the potential to significantly address the challenge of obtaining sufficient training data, a hurdle often encountered in deep learning-based Natural Language Processing techniques for procedure extraction.

==> background.tex <==


\subsection{Procedure definition}

In the following, we discuss a semantic representation of procedural knowledge in order to support various tasks. The representation should define the structure of procedures by specifying semantic elements of a procedure and their interrelated information. We propose a generic representation shown in Figure \ref{fig:procedure}, which, as we shall show, can support a number of tasks related to procedural knowledge. 


 \begin{figure*}[h!]
\centering
\begin{subfigure}{0.30\textwidth}
  \centering
  \includegraphics[width=\textwidth]{img/atomicProcedure.png}
  \caption{Atomic Procedure}
  \label{fig:atomicprocedure}
\end{subfigure}%
\begin{subfigure}{0.30\textwidth}
  \centering
  \includegraphics[width=\textwidth]{img/composteProcedure.png}
  \caption{Composed Procedure}
  \label{fig:composedprocedure}
\end{subfigure}
\caption{Atomic Procedure (left) and Composed Procedure (right).}
\label{fig:procedure}
\end{figure*}


\begin{definition}

A procedure $P$ that is executed can be defined as an ordered set of steps $S_1$, $\ldots$, $S_n$. A step $S_i$ is called a \textit{simple step} if it does not contain other finer-grained steps (sub-steps). Otherwise, it is referred to as a procedure. Each procedure consists of a starting and ending step with the former having no predecessors and the latter having no successors. 
A simple step $S_i$ can be further described with i) a set of \textit{actions} which represent the objectives of the activity; ii) a \textit{component} on which the activity takes place; iii) a \textit{tool} which carries out a particular function for performing the activity; iv) a \textit{product} or \textit{system} subject to the activity; and v) one or more \textit{quantifiers} that specify the temporal parameters (to describe the duration of activity), the spatial parameters (to describe the directional and location change) and quantitative parameters (to describe expressions of quantitative amount).
\end{definition}

\begin{definition}
    If the procedure performs a set of simple steps, the procedure is called \textit{atomic procedure}. 
\end{definition}

\begin{definition}
    If the procedure performs a set of steps that refer to other procedures, the procedure is called \textit{composed procedure}.
\end{definition}

%\textbf{Example}

This generic representation of procedures can be used to support different tasks related to procedural knowledge, such as documentation generation, procedural question answering and procedure automation.

\subsection{Procedure definition}

In the following, we discuss a semantic representation of procedural knowledge in order to support various tasks. The representation should define the structure of procedures by specifying semantic elements of a procedure and their interrelated information. We propose a generic representation shown in Figure \ref{fig:procedure}, which, as we shall show, can support a number of tasks related to procedural knowledge. 


 \begin{figure*}[h!]
\centering
\begin{subfigure}{0.30\textwidth}
  \centering
  \includegraphics[width=\textwidth]{img/atomicProcedure.png}
  \caption{Atomic Procedure}
  \label{fig:atomicprocedure}
\end{subfigure}%
\begin{subfigure}{0.30\textwidth}
  \centering
  \includegraphics[width=\textwidth]{img/composteProcedure.png}
  \caption{Composed Procedure}
  \label{fig:composedprocedure}
\end{subfigure}
\caption{Atomic Procedure (left) and Composed Procedure (right).}
\label{fig:procedure}
\end{figure*}


\begin{definition}

A procedure $P$ that is executed can be defined as an ordered set of steps $S_1$, $\ldots$, $S_n$. A step $S_i$ is called a \textit{simple step} if it does not contain other finer-grained steps (sub-steps). Otherwise, it is referred to as a procedure. Each procedure consists of a starting and ending step with the former having no predecessors and the latter having no successors. 
A simple step $S_i$ can be further described with i) a set of \textit{actions} which represent the objectives of the activity; ii) a \textit{component} on which the activity takes place; iii) a \textit{tool} which carries out a particular function for performing the activity; iv) a \textit{product} or \textit{system} subject to the activity; and v) one or more \textit{quantifiers} that specify the temporal parameters (to describe the duration of activity), the spatial parameters (to describe the directional and location change) and quantitative parameters (to describe expressions of quantitative amount).
\end{definition}

\begin{definition}
    If the procedure performs a set of simple steps, the procedure is called \textit{atomic procedure}. 
\end{definition}

\begin{definition}
    If the procedure performs a set of steps that refer to other procedures, the procedure is called \textit{composed procedure}.
\end{definition}

%\textbf{Example}

This generic representation of procedures can be used to support different tasks related to procedural knowledge, such as documentation generation, procedural question answering and procedure automation.




